Structure-Preserving Constrained Optimal Trajectory Planning of a Wheeled Inverted Pendulum

The Wheeled Inverted Pendulum (WIP) is an underactuated, nonholonomic mechatronic system, and has been popularized commercially as the Segway. Designing a control law for motion planning, that incorporates the state and control constraints, while respecting the configuration manifold, is a challenging problem. In this article we derive a discrete-time model of the WIP system using discrete mechanics and generate optimal trajectories for the WIP system by solving a discrete-time constrained optimal control problem. Further, we describe a nonlinear continuous-time model with parameters for designing a closed loop LQ-controller. A dual control architecture is implemented in which the designed optimal trajectory is then provided as a reference to the robot with the optimal control trajectory as a feedforward control action, and an LQ-controller in the feedback mode is employed to mitigate noise and disturbances for ensuing stable motion of the WIP system. While performing experiments on the WIP system involving aggressive maneuvers with fairly sharp turns, we found a high degree of congruence in the designed optimal trajectories and the path traced by the robot while tracking these trajectories. This corroborates the validity of the nonlinear model and the control scheme. Finally, these experiments demonstrate the highly nonlinear nature of the WIP system and robustness of the control scheme.

==> blockschaltbilder.tex <==
\newcommand{\Summationsstelle}[4][]{ %
  \begin{scope}[thick, #1]
    % Runder leerer Knoten mit vordefinierter Größe
    \node[draw, circle, minimum width = #4, minimum height = #4] (#2) at (#3) {};
  \end{scope} %
}

\newcommand{\Verzweigung}[4][]{ %
  \begin{scope}[inner sep = 0 pt, outer sep = 0 pt, thick, #1]
    % Leerer Knoten mit vordefinierter Größe
    \node[circle, minimum width = #4, minimum height = #4] (#2) at (#3) {};
    % Gefüllter Kreis
    \draw[solid, fill] (#2) circle (0.5*#4);
  \end{scope} %
}

\newcommand{\UeFunk}[5][]{ %
  \begin{scope}[thick, #1]
    % Knoten mit vordefinierter Größe
    \node[minimum width = #4, minimum height = #4] (#2) at (#3) {#5};
    % Block
    \draw (#2.north east) rectangle (#2.south west);
  \end{scope} %
}

\newcommand{\MGlied}[5][]{ %
  \begin{scope}[thick, #1]
    % Leerer Knoten mit vordefinierter Größe
    \node[minimum width = #4, minimum height = #4] (#2) at (#3) {};
    % Beschriftung über dem Block
    \node[fill = none, above, align = left, text width = #4] at (#2.north) {#5};
    % Block
    \draw (#2.north east) rectangle (#2.south west);
    % Multiplikationspunkt
    \draw[solid, very thin, fill] (#2.center) circle (0.11*#4);
  \end{scope} %
}

\newcommand{\MGliedVar}[5][]{ %
  \begin{scope}[thick, #1]
    % Leerer Knoten mit vordefinierter Größe
    \node[minimum width = #4, minimum height = #4] (#2) at (#3) {};
    % Beschriftung über dem Block
    \node[fill = none, above, align = left, text width = #4] at (#2.north) {#5};
    % Block
    \draw (#2.north east) rectangle (#2.south west);
    % Multiplikationskreuz
    \draw (#2.center) %
      +(45:0.225*#4) -- +(-135:0.225*#4) %
      +(-45:0.225*#4) -- +(135:0.225*#4);
  \end{scope} %
}

\newcommand{\PGlied}[5][]{ %
  \begin{scope}[thick, #1]
    % Leerer Knoten mit vordefinierter Größe
    \node[minimum width = #4, minimum height = #4] (#2) at (#3) {};
    % Beschriftung über dem Block
    \node[fill = none, above, align = left, text width = #4] at (#2.north) {#5};
    % Block
    \draw (#2.north east) rectangle (#2.south west);
    % Horizontale Linie
    \draw ([yshift = -0.225*#4] #2.north east) -- ([yshift = -0.225*#4] #2.north west);
  \end{scope} %
}

\newcommand{\IGlied}[5][]{ %
  \begin{scope}[thick, #1]
    % Leerer Knoten mit vordefinierter Größe
    \node[minimum width = #4, minimum height = #4] (#2) at (#3) {};
    % Beschriftung über dem Block
    \node[fill = none, above, align = left, text width = #4] at (#2.north) {#5};
    % Block
    \draw (#2.north east) rectangle (#2.south west);
    % Diagonale Linie
    \draw (#2.north east) -- (#2.south west);
  \end{scope} %
}

\newcommand{\DGlied}[5][]{ %
  \begin{scope}[thick, #1]
    % Leerer Knoten mit vordefinierter Größe
    \node[minimum width = #4, minimum height = #4] (#2) at (#3) {};
    % Beschriftung über dem Block
    \node[fill = none, above, align = left, text width = #4] at (#2.north) {#5};
    % Block
    \draw (#2.north east) rectangle (#2.south west);
    % D-Eck
    \draw ([xshift = 0.300*#4] #2.north west) |- ([yshift = 0.225*#4] #2.south east);
  \end{scope} %
}

\newcommand{\TZGlied}[6][]{ %
  \begin{scope}[thick, #1]
    % Leerer Knoten mit vordefinierter Größe
    \node[minimum width = #4, minimum height = #4] (#2) at (#3) {};
    % Beschriftung über dem Block
    % \mbox stellt sicher, dass \hfill auch bei fehlenden Argumenten aktiv ist
    \node[fill = none, above, align = center, text width = #4] at (#2.north) {\mbox{#5} \hfill \mbox{#6}};
    % Block
    \draw (#2.north east) rectangle (#2.south west);
    % Totzeit-Eck
    \draw ([xshift = 0.400*#4] #2.south west) |- ([yshift = -0.225*#4] #2.north east);
  \end{scope} %
}

\newcommand{\PTEinsGlied}[6][]{ %
  \begin{scope}[thick, #1]
    % Leerer Knoten mit vordefinierter Größe
    \node[minimum width = #4, minimum height = #4] (#2) at (#3) {};
    % Beschriftung über dem Block
    % \mbox stellt sicher, dass \hfill auch bei fehlenden Argumenten aktiv ist
    \node[fill = none, above, align = center, text width = #4] at (#2.north) {\mbox{#5} \hfill \mbox{#6}};
    % Block
    \draw (#2.north east) rectangle (#2.south west);
    % PT1-Kurve
    \begin{scope}[shift={(#2.south west)}]
      \draw %
        (0.00, 0.00) .. controls (0.10*#4, 0.80*#4) and (0.40*#4, 0.80*#4) .. %
        ([yshift = -0.18*#4] #2.north east);
    \end{scope} %
  \end{scope} %
}

\newcommand{\PTZweiGlied}[6][]{ %
  \begin{scope}[thick, #1]
    % Leerer Knoten mit vordefinierter Größe
    \node[minimum width = #4, minimum height = #4] (#2) at (#3) {};
    % Beschriftung über dem Block
    % \mbox stellt sicher, dass \hfill auch bei fehlenden Argumenten aktiv ist
    \node[fill = none, above, align = center, text width = #4] at (#2.north) {\mbox{#5} \hfill \mbox{#6}};
    % Block
    \draw (#2.north east) rectangle (#2.south west);
    % PT2-Kurve
    \begin{scope}[shift={(#2.south west)}]
      \draw %
        (0.00,    0.00   ) .. controls (0.07*#4, 0.00   ) and (0.10*#4, 0.10*#4) .. %
        (0.18*#4, 0.40*#4) .. controls (0.26*#4, 0.70*#4) and (0.35*#4, 0.85*#4) .. %
        (0.43*#4, 0.85*#4) .. controls (0.49*#4, 0.85*#4) and (0.58*#4, 0.75*#4) .. %
        (0.64*#4, 0.69*#4) .. controls (0.70*#4, 0.63*#4) and (0.76*#4, 0.59*#4) .. %
        (0.82*#4, 0.59*#4) .. controls (0.88*#4, 0.59*#4) and (0.97*#4, 0.60*#4) .. %
        ([yshift = -0.35*#4)] #2.north east);
    \end{scope} %
  \end{scope} %
}

\newcommand{\NeueEA}[5]{ %
  % Füge neue Koordinaten hinzu:
  % Nordseite (oben), von links nach rechts
  \foreach \i in {1, 2, ..., #2}
  {
    \coordinate (#1--north \i) at
      ($(#1.north west)!{(\i - 0.5)/(#2)}!(#1.north east)$);
  }
  % Ostseite (rechts), von oben nach unten
  \foreach \i in {1, 2, ..., #3}
  {
    \coordinate (#1--east \i) at
      ($(#1.north east)!{(\i - 0.5)/(#3)}!(#1.south east)$);
  }
  % Südseite (unten), von links nach rechts
  \foreach \i in {1, 2, ..., #4}
  {
    \coordinate (#1--south \i) at
      ($(#1.south west)!{(\i - 0.5)/(#4)}!(#1.south east)$);
  }
  % Westseite (links), von oben nach unten
  \foreach \i in {1, 2, ..., #5}
  {
    \coordinate (#1--west \i) at
      ($(#1.north west)!{(\i - 0.5)/(#5)}!(#1.south west)$);
  }
}

\newcommand{\KLGlied}[7][]{ %
  \begin{scope}[thick, #1]
    % Leerer Knoten mit vordefinierter Größe
    \node[minimum width = #4, minimum height = #4] (#2) at (#3) {};
    % Block
    \draw (#2.north east) rectangle (#2.south west);
    % Platz für die Kennlinie
    \begin{scope}[shift = {(#2.center)}, x = 0.4*#4, y = 0.4*#4]
      #5
    \end{scope}
    % Beschriftung über dem Block
    % \mbox stellt sicher, dass \hfill auch bei fehlenden Argumenten aktiv ist
    \node[fill = none, above, align = center, text width = #4] at (#2.north) {\mbox{#6} \hfill \mbox{#7}};
  \end{scope} %
}

\newcommand{\Saettigung}[6][]{ %
  \KLGlied[#1]{#2}{#3}{#4}{%
    \draw[thin, -latex] (0, -1) -- (0, 1);
    \draw[thin, -latex] (-1, 0) -- (1, 0);
    \draw[thick] (-1, -0.8) -- (-0.4, -0.8) -- (0.4, 0.8) -- (1, 0.8);
  }{#5}{#6}
}

